Parameterized Complexity of Path Set Packing

In Path Set Packing, the input is an undirected graph $G$, a collection $\calp$ of simple paths in $G$, and a positive integer $k$. The problem is to decide whether there exist $k$ edge-disjoint paths in $\calp$. We study the parameterized complexity of Path Set Packing with respect to both natural and structural parameters. We show that the problem is $W[1]$-hard with respect to vertex cover number, and $W[1]$-hard respect to pathwidth plus maximum degree plus solution size. These results answer an open question raised in COCOON 2018. On the positive side, we present an FPT algorithm parameterized by feedback vertex number plus maximum degree, and present an FPT algorithm parameterized by treewidth plus maximum degree plus maximum length of a path in $\calp$. These positive results complement the hardness of Path Set Packing with respect to any subset of the parameters used in the FPT algorithms. We also give a $4$-approximation algorithm for maximum path set packing problem which runs in FPT time when parameterized by feedback edge number.

==> algorithms.tex <==
\subsection{FPT algorithm parameterized by Treewidth $+$ Maximum Degree $+$ Maximum Path Length} \label{sec:3parameters}

Given a pair $(G,\calp)$, consider the auxiliary graph $H$ whose vertices correspond to paths in $\calp$ and in which two vertices are adjacent if the corresponding paths intersect at an edge. Then, finding the maximum path set packing in $\calp$ is equivalent to finding a maximum size independent set in $H$.
We can deduce the following facts about the structure of $H$.

\begin{lemma} \label{lemma:fpt}
If $G$ has treewidth $\tau$ and maximum degree $\Delta$, and each path in $\calp$ is of length at most $r$, then the treewidth of $H$ is at most $(\tau+1)\Delta^r$.
\end{lemma}

\begin{proof}
Given a tree decomposition $(T,\beta)$ of $G$ of width $\tau$, consider the pair $(T,\gamma)$, where $\gamma(v)=\cup_{x \in \beta(v)} \cup \{p\}$,
where the inner union is over all paths $p$ in $G$ of length at most $r$ and containing $x$.
We have $|\gamma(v)| \leq (\tau+1)\Delta^{r}$ since each vertex in $\beta(v)$ belongs to at most $\Delta^{r}$ paths of length at most $r$ in $G$. Further $(T,\gamma)$ is a tree decomposition of $H$: 

(a) for every $p\in \calp$, there exists a node $v$ in $T$ such that $p$ is in $\gamma(v)$, eg: node $v\in V(T)$ such that $\beta(v)$ contains a vertex of $p$;

(b) if $p,q\in \calp$ are adjacent in $H$ that is $p,q$ intersect at an edge, then both $p,q$ belong to $\gamma(v)$ for a node $v$ in $T$ such that $\beta(v)$ contains a common vertex of $p,q$;

(c) now we show that for every $p \in \calp$, the set of all the nodes $v\in V(T)$ such that $\gamma(v)$ contains $p$ induces a connected subgraph of $T$.
We assume to the contrary that there is a path $p \in \calp$ such that the set $S(p)$ of all the nodes in $T$ such that $\gamma(v)$ contains $p$ does not induce a connted subgraph of $T$, then there must be a node $v$ in $T$ such that $p \notin \gamma(v)$ and $v$ belongs to the path between two distinct nodes in $S(p)$ which belong to separate components in $T[S(p)]$. Graph $G-\beta(v)$ is disconnected
and has at least two connected components containing two distinct vertices, say $x,y$ of the path $p$. This implies that at least one vertex of the subpath of $p$ joining $x,y$ must belong to $\beta(v)$, and thus $p$ belongs to $\gamma(v)$, a contra position to our assumption.
\qed
\end{proof}

The Maximum Independent Set problem admits a $O(2^{\tau})$ algorithm on graphs of treewidth $\tau$ \cite{AP89}.
Hence we obtain Theorem \ref{theorem:tw_maxdegree} as a corollary.


